Robust Prompt Optimization for Defending Language Models Against Jailbreaking Attacks

Despite advances in AI alignment, large language models (LLMs) remain vulnerable to adversarial attacks or jailbreaking, in which adversaries can modify prompts to induce unwanted behavior. While some defenses have been proposed, they have not been adapted to newly proposed attacks and more challenging threat models. To address this, we propose an optimization-based objective for defending LLMs against jailbreaking attacks and an algorithm, Robust Prompt Optimization (RPO) to create robust system-level defenses. Our approach directly incorporates the adversary into the defensive objective and optimizes a lightweight and transferable suffix, enabling RPO to adapt to worst-case adaptive attacks. Our theoretical and experimental results show improved robustness to both jailbreaks seen during optimization and unknown jailbreaks, reducing the attack success rate (ASR) on GPT-4 to 6% and Llama-2 to 0% on JailbreakBench, setting the state-of-the-art. Code can be found at https://github.com/lapisrocks/rpo

==> secs/impact_statement.tex <==
This paper's goal is to advance the field of machine learning by improving the safety and robustness of language models, specifically under adversarial conditions. As language models improve in capabilities and are increasingly deployed in real-world contexts, ensuring safety becomes crucial. Our proposed method can empirically improve robustness to jailbreaking attacks, an important security vulnerability of many LMs. RPO is also designed with practical applications in mind. We show that RPO suffixes can easily transfer across models, are easy to use, and have a minimal effect on benign prompts.

However, proposing our defense method may lead to the development of new attacks, including attacks that can break RPO. Additionally, we release example attack prompts in this paper for reproducibility, which could potentially be used to attack models. However, these prompts are also publicly available online, and our results suggest that preventing jailbreaking on LMs is a tractable problem. 

We hope our work highlights the vulnerabilities of LMs and motivates additional work in this direction. A full analysis of our proposed objectives, such as robustness certifications or adversarial risk bounds, would strengthen confidence in the effectiveness of RPO. We expect both attacks and LMs to adapt and evolve, which will also force threat models to change. For instance, the latest version of GPT-4 also supports visual inputs, which is unsupported by our threat model. More robust defenses may require adversarial training, more extensive red-teaming, or stronger discrete optimization algorithms. In addition, In the broader context of trustworthy machine learning, we encourage research towards ensuring powerful models such as LMs remain harmless in all contexts. While our paper focuses on harmful generation, we urge a larger analysis and mitigation of failure modes, such as truthfulness and bias. In addition, as models improve, we expect additional failure modes to emerge and encourage further research in further understanding and mitigating the potential risks of LMs and other powerful models. 

==> secs/method.tex <==
\hw{
\subsection{Background}
math of adversarial examples and adversarial training
}


\subsection{Threat Model}

We are interested in robustness from an \textit{alignment} perspective, in which unwanted behavior can be broader and more harmful than misclassification. We conduct our study around a \textit{threat model}, which allows us to consider realistic scenarios and formalize our objectives. By doing so, we can more accurately evaluate LM robustness under worst-case scenarios or the presence of adversaries. We assume the adversary has white-box access to some models and black-box API access to others. To encompass the expanding list of possible jailbreaks, we assume the adversary can freely select various jailbreaks until the attack is successful. This is a more difficult threat model than what is explored in previous work, as we find that the nature of prompting significantly reduces the difficulty of conducting more than a single type of attack compared to vision. Consequently, we focus on the \textit{multiattack robustness} setting \cite{tramèr2019adversarial,maini2020adversarial,dai2023multirobustbench} and aim to create defenses robust to multiple jailbreaks, similar to perceptual adversarial robustness \cite{laidlaw2021perceptual} in vision. We expect threat models to evolve as techniques to create attacks improve.

Defining a threat model also allows us to build effective defenses, which we propose should include the following criteria. \textit{Universality}. Due to the amount of possible jailbreaks, defenses should improve robustness broadly instead of on a single attack. \textit{Practicality}. As language models are widely deployed, a good defense should be cheap and not compromise general usefulness. \textit{Effectiveness}. A good defense should improve robustness in worst-case scenarios, such as unknown attacks to which the base model is completely vulnerable.

% \az{The only "constraint" is the GCG suffix length which we match. Do we need to mention this?}

\subsection{Attack Objective}
\hwc{never mentioned notations?}

The goal of an adversary is to induce a language model to respond to \textit{any} request, including harmful ones the model would normally reject. We consider a standard autoregressive language model where a sequence of tokens is mapped to the distribution over the next token. This objective can be formulated as 
\begin{equation}
    p(x_{n+1} | x_{1:n}),
\end{equation}
which denotes the probability that the next token is $x_{n+1}$ given previous tokens $x_{1:n}$. We use $p(y | x_{1:n})$ to denote the probability of generating every token in the output sequence $y$ given all previous tokens to that point.
\begin{equation}
    p(y~|~x_{1:n}) = \prod_{i=1} p(x_{n+i} | x_{1:n+i-1})
\end{equation}

We consider a modern language model optimized to produce outputs that match human preferences \cite{ziegler2019finetuning,bai2022training,rafailov2023direct}, which is described as a latent reward model $r^*(y | x_{1:n})$ where a high reward is given to outputs more aligned with human evaluations. In the context of jailbreaking, $x_{1:n}$ is a harmful instruction such as "How do I build a bomb," which we denote as $\hat{x}_{1:n}$.

We consider the setting where the adversary can modify $\hat{x}_{1:n}$ through either manual jailbreaks or gradient-based jailbreaks to maximize the probability of producing an output sequence that accepts the harmful request or is toxic. This can be formulated as the negative log probability of the target sequences of tokens $y^\star$ representing the worst-case output $y^\star = \min r^*(y | \hat{x}_{1:n})$, which results in the following adversarial loss and optimization objective of the adversary,
\begin{equation}
\label{eq:generation-loss}
    \mathcal{L}^{adv}(\hat{x}_{1:n}) = -\log p(y^\star | \hat{x}_{1:n}).
\end{equation}
\begin{equation}
\label{eq:adversarial-objective}
\minimize \mathcal{L}^{adv}(\hat{x}_{1:n}).
\end{equation}
% \hwc{why is this adv loss, is it because the $x^\star$ has some special property? what are these properties}

In practice, Obj \ref{eq:adversarial-objective} is optimized through modifications to $\hat{x}_{1:n}$. We focus on the gradient-based attack GCG \cite{zou2023universal}, which directly optimizes the objective by replacing tokens in a suffix with ones that minimize the loss, and manual jailbreaks \cite{Wei2023JailbrokenHD} consisting of various human-designed prompts.

\subsection{Defense Objective}

While prevailing methods to improve LM alignment involve fine-tuning \cite{christiano2017deep, rafailov2023direct}, the objective of matching human preferences does not directly account for worst-case scenarios where an adversary is introduced. In addition, the high cost of generating adversarial suffixes makes adversarial training on these samples infeasible \cite{jain2023baseline}. We center our approach on the \textit{prompt} level to address this. Not only does this reduce the risk of changing the base model, but the tendency of LMs to already refuse harmful instructions indicates it is possible to steer it toward harmless behavior with only modifications to the prompt. We formalize this as the negative log probability of a target token output $y^\prime$ that refuses $\hat{x}_{1:n}$. This can be represented as the normal output of an LM trained to maximize $r^\prime$ or $y^\prime = \max r^*(y | \hat{x}_{1:n}) $, resulting in the safe loss and defense objective,
\begin{equation}
\label{eq:generation-loss-safe}
    \mathcal{L}^{safe}(\hat{x}_{1:n}) = -\log p(y^\prime | \hat{x}_{1:n})
\end{equation}
\begin{equation}
\label{eq:defense-objective}
\minimize \mathcal{L}^{safe}(\hat{x}_{1:n}).
\end{equation}
% \hwc{similarly, eq (3) and eq(5) are mathematically the same with different notations, what is the actual thing that makes them different and what are the mathematical descriptions of that thing?}

This objective is often indirectly optimized for through the inclusion of \textit{system prompts}, inputs to the LM the user or adversary cannot alter. System prompts tell the LM to act a certain way, such as "You are a harmless and helpful assistant."

The goal of the defense objective is to ensure robustness even under worst-case scenarios, such as when a jailbreak alters the harmful prompt. This can be formalized by incorporating the adversary into Obj \ref{eq:defense-objective}, which yields the following objective,

\begin{equation}
\label{eq:joint-objective}
\minimize \mathcal{L}^{safe}(\minimize \mathcal{L}^{adv}(\hat{x}_{1:n})).
\end{equation}


\begin{algorithm*}[t]
    \caption{Robust Prompt Optimization}
    \label{alg:universal-opt}
    \begin{algorithmic}
    \Require Prompts $x_{1:n_1}^{(1)} \ldots\, x_{1:n_m}^{(m)}$, set of jailbreaks $\mathcal{A}$, initial defensive suffix $p_{1:l}$, losses $\mathcal{L}_1^{\text{safe}} \ldots, \mathcal{L}_m^{\text{safe}}$, iterations $T$, $k$, batch size $B$, selection interval $R$

    \For{$s = 1,\ldots,S$} 
        \Loop{ $T$ times}
            \ForAll{prompts $x_{1:n_1}^{(1)} \ldots\, x_{1:n_m}^{(m)}, j = 1\ldots m$ }
            \State Append defensive suffix $p_{1:l}$ to $x_{1:n_i}^{(j)}$
                \If{$t \mod R == 0$} \Comment{Apply selection every $R$ steps}
                    \State $A^* := \argmin_{\mathcal{A}} \mathcal{L}_j^{\text{adv}}\sum_{1 \le o \le m}(A_o(x^{(j)}))$ \Comment{Select jailbreak that minimizes adversarial loss}
                    \State $x^{(j)} := A^*(x^{(j)})$ \Comment{Apply best jailbreak from set to prompt}
                \EndIf
                    \EndFor
                    \For{$i \in [0 \ldots l]$}
                        \State $\mathcal{X}_i := \mbox{Top-}k(-\sum_{1 \le j \le m} \nabla_{e_{p_i}} \mathcal{L}_j^{\text{safe}}(x_{1:n+l}^{(j)}\|p_{1:l}))$\Comment{Compute top-k candidates}
                    \EndFor
                    \For{$b = 1,\ldots,B$}
                        \State $\tilde{p}_{1:l}^{(b)} := p_{1:l}$ 
                        \State
                        $\tilde{p}_{1:l}^{(b)} := \mbox{Uniform}(\mathcal{X}_i)$ \Comment{Sample replacements}
                    \EndFor
                    \State $p_{1:l} := \tilde{p}^{(b^\star)}_{1:l}$, where $b^\star = \argmin_b \sum_{1 \le j \le m}\mathcal{L}_j^{\text{safe}}(x^{(j)}_{1:n+l}\|\tilde{p}^{(b)}_{1:l})$ \Comment{Compute best replacement}
        \EndLoop
    \EndFor
    \Return Optimized defensive suffix $p$
    \end{algorithmic}
    \end{algorithm*}

Like adversarial training, this formulation can be viewed as the composition of two problems, an \textit{inner minimization} problem, and \textit{outer minimization} problem. Both manual and gradient-based jailbreaks can be interpreted as methods to solve the inner minimization problem by creating a prompt to minimize the adversarial loss, while recently proposed defenses that modify the prompt with smoothing \cite{Robey2023SmoothLLMDL} or few-shot examples \cite{Zhang2023DefendingLL} indirectly solve the outer minimization problem.

Our main technical contribution is a method that directly optimizes this objective, yielding a prompt more robust to both manual and gradient-based jailbreaks.


\subsection{Robust Prompt Optimization}

% We use existing attacks such as GCG \cite{zou2023universal} and manual jailbreaks from \cite{Wei2023JailbrokenHD} to solve the inner minimization part of the optimization objective. To complete the optimization, we propose the first method to solve the outer minimization problem directly and optimize for \ref{eq:joint-objective}. 

In this section, we describe our proposed method to solve Obj \ref{eq:joint-objective}. Without direct gradient updates to the LM, we focus on input optimization, which is challenging for LMs due to the discrete nature of text. Existing techniques generally fall under two categories: \textit{semantic modifications}, often with an LM \cite{pryzant2023automatic} or RL policy \cite{deng-etal-2022-rlprompt}, and \textit{token optimization} using gradients \cite{autoprompt:emnlp20}. The strongest jailbreaks also adopt similar optimization methods, such as genetic algorithms \cite{liu2023autodan}, gradient-based optimization \cite{zou2023universal}, and semantic modifications with an LM \cite{mehrotra2023tree,anonymous2024quack}. 

We find that in this setting, semantic modifications, while semantically meaningful, are limited to simple operations such as rephrasing and do not modify the base prompt well enough to defend against more than a few jailbreaks. Generally, these optimization methods can enhance the effectiveness of an already successful prompt but cannot discover new prompt designs on their own. Intuitively, it is also unlikely that there will be a particular system prompt that can defend against jailbreaking universally due to the sheer volume of possible exploits. In addition, semantic operations can be exploited by iterative, adaptive attacks such as GCG \cite{zou2023universal}, or AutoDAN \cite{liu2023autodan}. 

Due to these limitations, we focus on gradient-based token optimization, which can \textit{directly} optimize for Obj \ref{eq:joint-objective}. In general, solving this objective means creating a mapping between \textit{any} worst-case modification of the input or jailbreak and the distribution of normal responses with the original prompt. This can be achieved by optimizing a suffix that always results a harmless output. To do so, we propose our main algorithm, \textit{robust prompt optimization (RPO)}, which optimizes for a set of tokens to enforce this mapping. As a whole, RPO consists of two components based on the two components of the overall objective: (1) a jailbreak selection step that applies a worst-case modification to the prompt and (2) a discrete optimization step that modifies a suffix to maintain a harmless output.

We simulate the adaptive threat model for the first component and apply a jailbreak to the original prompt under the addition of the current defensive suffix. This is a straightforward modification to the prompt for simple, manual jailbreaks. For gradient-based or iterative jailbreaks such as GCG \cite{zou2023universal} or AutoDAN \cite{liu2023autodan}, we apply one iteration of the jailbreak to reduce cost. Our main technical contribution for this component is the selection step, where we select from our training set the jailbreak that minimizes the adversarial loss for that prompt, according to Obj \ref{eq:adversarial-objective}. This ensures the optimization is performed under worst-case conditions and reduces the chance for a suffix to overfit on a particular jailbreak. We also jointly optimize over multiple prompts, which contain various harmful instructions. In practice, due to the cost of evaluating the adversarial loss, we only perform this operation after a certain number of iterations and otherwise keep the same jailbreak for each prompt.

After a jailbreak is applied, the second component optimizes the suffix to minimize the safe loss Obj \ref{eq:defense-objective}. We adopt a method similar to GCG, using a greedy coordinate descent approach to assess how replacing the \textit{i}-th token affects the safe loss. This involves calculating the first-order approximation and selecting the top-\textit{k} tokens with the largest negative gradient. We then randomly select $B \leq k |\mathcal{I}|$ tokens from this set of candidates, obtain the exact loss on this subset, and replace the current token with the token with the smallest loss. This process is conducted until a set number of iterations $T$ is reached. The full algorithm is described in Alg \ref{alg:universal-opt}.

% The key distinction from GCG is that we integrate this procedure with a jailbreak. For manual jailbreaks, which are static in our setting, this is essentially GCG with a target output refusing the instruction. However, due to the vast space of possible natural language jailbreaks, we find that the resulting suffix does not transfer to other jailbreaks well. Instead, we focus on optimizing against the GCG attack, which is more adaptive. This results in two suffixes to optimize, an \textit{adversarial suffix} and a \textit{defensive suffix}. To solve this, we propose a discrete optimization algorithm, \textit{robust prompt optimization}, which jointly optimizes for both suffixes. During every iteration, we replace tokens in each suffix in succession. When a suffix is optimized, the other is placed in the context of the LM, which allows the gradients to take the other suffix into account. We optimize until a set number of iterations $T$ is reached. 

% To optimally solve for \ref{eq:joint-objective}, the adversarial suffix must sufficiently explore the space of possible suffixes, which is challenging for discrete optimization. Not only is the space of suffixes combinatorial and unbounded, but the gradients are also biased to the existing string and tend to become stuck in local minima. To help with this, we find that using random restarts or resetting the adversarial suffix to another reduces overfitting. The full algorithm is described in \ref{alg:universal-opt}. 

    % \begin{algorithm*}[!h]
    % \caption{Robust Prompt Optimization (Multiattack)}
    % \label{alg:universal-opt}
    % \begin{algorithmic}
    % \Require Prompts $x_{1:n_1}^{(1)} \ldots\, x_{1:n_m}^{(m)}$, jailbreaks $J^{1}\ldots\, J^{n}$, adversarial suffixes $g_{1:l}^{(1)} \ldots\, g_{1:l}^{(S)}$, initial defensive suffix $p_{1:l}$, losses $\mathcal{L}_1^{\text{safe}} \ldots, \mathcal{L}_m^{\text{safe}}$, $\mathcal{L}_1^{\text{adv}} \ldots, \mathcal{L}_m^{\text{adv}}$,iterations $T$, $k$, batch size $B$
    % \For{$s = 1,\ldots,S$} 
    %     \State $g := g^s$ \Comment{Start with first suffix}
    %     \Loop{ $T$ times}
    %         \State Append adversarial suffix $g_{1:l}$ to each prompt in $x_{1:n_1}^{(1)} \ldots\, x_{1:n_m}^{(m)}$

    %         \For{$i \in [0 \ldots l]$}
    %             \State $\mathcal{X}_i := \mbox{Top-}k(-\sum_{1 \le j \le m} \nabla_{e_{p_i}} \mathcal{L}_j^{safe}(x_{1:n+l}^{(j)}\|p_{1:l}))$ 
    %             \Comment{Compute top-$k$ substitutions}
    %         \EndFor
    %         \For{$b = 1,\ldots,B$}
    %             \State $\tilde{p}_{1:l}^{(b)} := p_{1:l}$
    %             \State $\tilde{p}^{(b)}_{i} := \mbox{Uniform}(\mathcal{X}_i)$, where $i = \mbox{Uniform}(\mathcal{I})$  
    %             \Comment{Select random substitute token}
    %         \EndFor
    %         \State $p_{1:l} := \tilde{p}^{(b^\star)}_{1:l}$, where $b^\star = \argmin_b \sum_{1 \le j \le m_c}\mathcal{L}_j^{safe}(x^{(j)}_{1:n+l}\|\tilde{p}^{(b)}_{1:l})$ 
    %         \Comment{Compute best replacement}

    %         \bigskip
    %         \bigskip

    %         \State Remove adversarial suffix and append postfix $p_{1:l}$ to each prompt in $x_{1:n_1}^{(1)} \ldots\, x_{1:n_m}^{(m)}$
    %         \For{$i \in [0 \ldots l]$}
    %             \State $\mathcal{X}_i := \mbox{Top-}k(-\sum_{1 \le j \le m} \nabla_{e_{p_i}} \mathcal{L}_j^{adv}(x_{1:n+l}^{(j)}\|g_{1:l}))$ 
    %             \Comment{Compute top-$k$ substitutions}
    %         \EndFor
    %         \For{$b = 1,\ldots,B$}
    %             \State $\tilde{g}_{1:l}^{(b)} := g_{1:l}$
    %             \State $\tilde{g}^{(b)}_{i} := \mbox{Uniform}(\mathcal{X}_i)$, where $i = \mbox{Uniform}(\mathcal{I})$  
    %             \Comment{Select random substitute token}
    %         \EndFor
    %         \State $g_{1:l} := \tilde{g}^{(b^\star)}_{1:l}$, where $b^\star = \argmin_b \sum_{1 \le j \le m_c}\mathcal{L}_j^{adv}(x^{(j)}_{1:n+l}\|\tilde{g}^{(b)}_{1:l})$ 
    %         \Comment{Compute best replacement}
    %     \EndLoop
    % \EndLoop
    % \Ensure Optimized defensive suffix $p$
    % \end{algorithmic}
    % \end{algorithm*}





% \subsection{Multiattack RPO}

% We observe that using RPO to optimize suffixes to defend against particular jailbreaks is effective and transfers to other jailbreaks, especially of similar types. For instance, a suffix optimized on a manual jailbreak will transfer well to other manual jailbreaks but not to gradient-based attack GCG \cite{zou2023universal}. Similarly, RPO suffixes optimized on GCG will transfer well to held-out GCG suffixes but less to manual jailbreaks. While this is rarely a requirement in vision, the ideal defense should exhibit universality to various jailbreaks, including unknown ones. To address this, we propose our main and most effective variant of RPO, an algorithm that aims to create a universal defense against prompt-level adversarial modifications. 

% We also propose a variant of RPO that can be optimized over various jailbreaks simultaneously.

==> tables/general_evals.tex <==
\begin{table}[t]
  \centering
  \footnotesize
  \caption{General LM evaluations after an RPO suffix is applied. We use the suffix optimized on Starling-7B \cite{starling2023} for all models for a fair comparison. AlpacaEval \cite{alpaca_eval} measures win-rate against human annotations on 20k prompts. We observe a small reduction in AlpacaEval performance, which decreases with larger models.}
    \begin{tabular}{l|l|ccc}
    \toprule
    Model & Method & MT-Bench & MMLU \\
    \midrule
    \multirow{2}{*}{Llama2-7B} & Base & 6.18 & 0.46 \\
    & RPO & 6.05 & 0.46 \\
    \midrule
    \multirow{2}{*}{Vicuna-13B} & Base & 6.57 & 0.50\\
    & RPO & 5.96 & 0.49 \\
    \midrule
    \multirow{2}{*}{GPT-3.5} & Base & 8.32 & 0.68 \\
    & RPO & 7.81 & 0.66 \\
    \midrule
    \multirow{2}{*}{GPT-4} & Base & 9.32 & 0.85 \\
    & RPO & 9.20 & 0.85 \\
    \bottomrule
    \end{tabular}
\end{table}


==> tables/gpt.tex <==
\begin{table*}
  \centering
  \caption{Attack Success Rate of GCG \citet{zou2023universal} and Adversarial Instructions \cite{Wei2023JailbrokenHD}, and Role-Playing \cite{Wei2023JailbrokenHD} for black-box GPT-4 \cite{openai2023gpt4}. We use the multiattack RPO suffix optimized on Starling-7B \cite{starling2023} from \ref{tab:individual} and apply it to each jailbreak. Base GPT-4 has low robustness but can easily follow safety-oriented instructions and defend against many strong jailbreaks. However, these manual defenses fail under adaptive attack GUARD \cite{jin2024guard}, which optimizes a manual jailbreak directly on GPT-4 with a knowledge graph. We find that RPO suffixes transfer to GPT-4 even on this difficult jailbreak.}
    \begin{tabular}{l|ccccc|cc}
    \toprule
    Method & Base & GCG & Adv Instructions & Role-Playing & GUARD & AlpacaEval $\uparrow$ & Add. Tokens $\downarrow$\\
    \midrule
    Base & 0.0 & 28.0 & 84.0 & 80.0 & 92.0 & 95.28 & 0 \\
    Perplexity Filter & 0.0 & 0.0 & 84.0 & 80.0 & 92.0 & 95.28 & 0\\
    Self-Reminder & 0.0 & 0.0 & 0.0 & 0.0 & 92.0 & 93.79 & 54 \\
    Goal Prioritization & 0.0 & 0.0 & 0.0 & 0.0 & 86.0 & 83.83 & 355 \\
    RPO (Ours) & 0.0 & 0.0 & 0.0 & 0.0 & 20.0 & 94.29 & 20 \\
    + In-Context Learning & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{6.0} & 81.84 & 375 \\
    \bottomrule
    \end{tabular}
  \label{tab:gpt}
  \vspace{-0.1in}
\end{table*}

==> tables/llama2.tex <==
\begin{table*}[t]
  \centering
  \caption{Attack Success Rate of GCG \citet{zou2023universal} and Adversarial Instructions \cite{Wei2023JailbrokenHD}, and Role-Playing \cite{Wei2023JailbrokenHD}. Under white-box attacks, the defensive suffix is optimized for each model and across all jailbreaks. Model is Llama2-7B-Chat \cite{touvron2023llama}. On test instructions, the single optimized suffix can fully defend against the role-playing attacks and dramatically improves robustness to the adversarial instructions.}
    \begin{tabular}{l|ccccc}
    \toprule
    Method & Base & GCG & Adv Instructions & Single-RolePlay & Multi-RolePlay \\
    \midrule
    Base & 0.0 & 84.0 & 50.0 & 10.0 & 20.0 \\
    Perplexity Filter {\scriptsize~\cite{jain2023baseline}} & 0.0 & 0.0 & 50.0 & 10.0 & 20.0 \\
    Goal Prioritization {\scriptsize~\cite{Zhang2023DefendingLL}} & 0.0 & 0.0 & 38.0 & 6.0 & 16.0 \\
    RPO ($l=20$) & 0.0 & 0.0 & 22.0 & 0.0 & 4.0 \\
    RPO ($l=40$) & 0.0 & 0.0 & 10.0 & 0.0 & 0.0 \\
    \bottomrule
    \end{tabular}
  \label{tab:llama}
\end{table*}

%RPO (Ours) & 0.0 & 2.0 & 4.0 & 0.0\\
  %  + In-Context Learning \cite{lin2023unlocking} & 0.0 & 0.0 & \textbf{0.0} & 0.0 \\

==> tables/llms.tex <==
\begin{table*}[t]
  \centering
  \caption{Attack Success Rate comparison across Llama-2-Chat \cite{touvron2023llama} models and Vicuna-7B \cite{zheng2023judging}. The table includes results for GCG \cite{zou2023universal}, Adversarial Instructions \cite{Wei2023JailbrokenHD}, and Role-Playing \cite{Wei2023JailbrokenHD}. We use the RPO suffix optimized on Starling-7B \cite{starling2023} and directly it on these models. RPO suffixes transfer well to alignment-trained LLama2-7B and LLama2-70B, and model trained on only instruction-following Vicuna-7B.}
    \begin{tabular}{l|l|cccc}
    \toprule
    Model & Method & Base & Adv Instructions & Single-RolePlay & Multi-RolePlay \\
    \midrule
    \multirow{3}{*}{Llama2-7B} & Base & 0.0 & 50.0 & 10.0 & 20.0 \\
    & Goal Prioritization & 0.0 & 38.0 & 6.0 & 16.0 \\
    & RPO (Ours) & \textbf{0.0} & \textbf{16.0} & \textbf{0.0} & \textbf{0.0} \\
    \midrule
    \multirow{3}{*}{Vicuna-7B} & Base & 12.0 & 68.0 & 28.0 & 60.0 \\
    & Goal Prioritization & 4.0 & \textbf{0.0} & 20.0 & 36.0  \\
    & RPO (Ours)  & \textbf{2.0} & 20.0 & \textbf{8.0} & \textbf{24.0} \\
    \midrule
    \multirow{3}{*}{Llama2-70B} & Base & 0.0 & 52.0 & 4.0 & 46.0 \\
    & Goal Prioritization  & 0.0 & 40.0 & 0.0 & 42.0 \\
    & RPO (Ours) & \textbf{0.0} & \textbf{24.0} & \textbf{0.0} & \textbf{2.0} \\
    \bottomrule
    \end{tabular}
  \label{tab:llms}
  \vspace{-0.1in}
\end{table*}

